Democratic Value and Money for Decentralized Digital Society

Classical monetary systems regularly subject the most vulnerable majority of the world's population to debilitating financial shocks, and have manifestly allowed uncontrolled global inequality over the long term. Given these basic failures, how can we avoid asking whether mainstream macroeconomic principles are actually compatible with democratic principles such as equality or the protection of human rights and dignity? This idea paper takes a constructive look at this question, by exploring how alternate monetary principles might result in a form of money more compatible with democratic principles -- dare we call it "democratic money"? In this alternative macroeconomic philosophy, both the supply of and the demand for money must be rooted in people, so as to give all people both equal opportunities for economic participation. Money must be designed around equality, not only across all people alive at a given moment, but also across past and future generations of people, guaranteeing that our descendants cannot be enslaved by their ancestors' economic luck or misfortune. Democratic money must reliably give all people a means to enable everyday commerce, investment, and value creation in good times and bad, and must impose hard limits on financial inequality. Democratic money must itself be governed democratically, and must economically facilitate the needs of citizens in a democracy for trustworthy and unbiased information with which to make wise collective decisions. An intriguing approach to implementing and deploying democratic money is via a cryptocurrency built on a proof-of-personhood foundation, giving each opt-in human participant one equal unit of stake. Such a cryptocurrency would have both interesting similarities to, and important differences from, a Universal Basic Income (UBI) denominated in an existing currency.

==> money/jackson.tex <==

\xxx{
Anyone who believes that exponential growth can go on forever
in a finite world is either a madman or an economist. 
-- Kenneth Boulding, 1973

‘[The GDP] measures everything… except that which makes life
worthwhile.’
Robert Kennedy, 1968
}

\com{
Notes from Tim Jackson, Prosperity Without Growth:

Through both peak and trough, the under- lying physical resource base moved inexorably towards exhaustion. The market is just too self-obsessed to measure this.p.10

The idea of a non-growing economy may be an anathema to an economist. But the idea of a continually grow- ing economy is an anathema to an ecologist. No subsystem of a finite system can grow indefinitely, in physical terms. Economists have to be able to answer the question of how a continually growing economic system can fit within a finite ecological system. p.14

...


---
Tim Jackson, The Post-growth Challenge

‘The question then arises,’ wrote Summers in 2014, ‘can we identify any
stretch during which the economy grew satisfactorily under conditions that
were financial sustainable?.’ 20 His answer, and indeed the answer of a
number of other economists, was: no. p.10

[On the financial bailout]
No one pretended this was anything other than a short-term solution. Many
even accepted that it was potentially regressive: a temporary fix that
rewarded those responsible for the crisis at the expense of the taxpayer. But
it was excused on the grounds that the alternative was simply unthinkable. p.11

The broad point is that the rate of labour productivity growth tells us
something fundamental about the capacity of the economy to deliver
income growth. It is central to our understanding of how hard people have
to work in order to sustain a given income level. p.14

The only way to squeeze economic growth out of an
economy with virtually no productivity growth at all is to have a higher
workforce participation or to have people working longer hours. p.16

[Clear explanation of "rich get richer" effects in today's economy]
There are several channels through which this acceleration of inequality
occurs. [...] p.23

Policy responses which attempt to
stimulate investment by reducing the interest rate, end up making money
cheaper and incentivising more speculation, fuelling a vicious cycle of rising
inequality. p.24

The dynamics of the existing growth based
paradigm are driving environmental damage, exacerbating social
inequality and contributing to increased political instability. There has
never been a more urgent need to question the growth imperative. There has
never been a more opportune time to develop the design concepts for a
resilient post-growth society. p.32


XXX Further reading:
See for example, D’Alisa et al 2014, van den Bergh 2015, Kallis 2015, Jackson 2017, Victor 2018. 
On UBI: See for instance: DiEM25 2017; RSA 2015; Peston 2017. 


Tim Jackson, Confronting inequality in a post-growth world

Piketty’s own suggestion for combatting systemic inequality is a tax on
capital assets (Piketty 2014)

we adopted a proposal similar to
those suggested by Wright (2005) and Varoufakis (2016) in which universal
basic income is funded through a social dividend paid from the ownership
of ‘common stock’

Mazzucato (2015) has
famously pointed out that every key innovation in Apple’s iPhone was
funded by the US government. The assumption that only Apple’s
shareholders should benefit from profits on sales of the iPhone is therefore
a distortion of the social contract in favour of the owners of capital and
against the interests of the public. 


XXX Further reading:
So, for example, any future movement towards a ‘secular stagnation’
(Gordon 2016, Summers 2015) is likely to be associated with even greater
inequality. Equally, any policies aimed at a ‘post-growth’ society (Blewitt
and Cunningham 2014, d’Alisa et al 2015, Cassiers et al 2017, Jackson 2018)
might have undesirable social outcomes. Certainly, the prospects for
‘prosperity without growth’ (Jackson 2009 & 2017) or ‘managing without
growth’ (Victor 2008 & 2018)

concept of a universal basic income (Gorz 1999, RSA 2015, Taylor 2017). 
 (Meade 1988, Gorz 1999, McKay 2001, Wright 2005) 
 (Murray 2008, JRF 2015, RSA 2015, Varoufakis 2016)

a potential
response to the threat of increased automation and declining job security
(Frase 2016, Varoufakis 2016, Pulkka 2017). 

fascinating insight into the structural dynamics through which capitalism
has an in-built function for the divergence of incomes (Kalecki 1939, Kaldor
1955, Galbraith 2013).


Jackson, "Motivating Sustainable Consumption", jackson05motivating:
extensive survey intended for policymaker audience on
theories and models of consumer behavior,
and theory and practice of policy-driven behavioral change,
with a focus on sustainability goals.

}%com




==> money/notes.tex <==
\com{	"This Time is Different"

Inflation Crises: discusses threshold of "pernicious" inflation:
prior studies often used 40%; this book uses 20%;
relatively insensitive from 15% to 25%.

The French finance minister Abbe Terray, who served from 1768 to 1774,
even opined that governments should default at least once every hundred years
in order to restore equilibrium. 2
[Winkler (1933), p. 29.
And Thomas Jefferson, "the tree of liberty must be refreshed from time to time
with the blood of patriots and tyrants." ]

Mississippi and South Sea bubbles memorialized in Charles Kindleberger's
classic book on bubbles, manias, and panics.
[Kindleberger (1989)]

}%com

\com{	"Ideas for Sufficiency" - riccardo mastini & leida rijnhout
	(Friends of the Earth Europe)	mastini18ideas
% http://www.foeeurope.org/sites/default/files/resource_use/2018/foee_sufficiency_booklet.pdf

The basic principle of
intragenerational equity entails that wealthy households in all
countries should consume less to free up the ‘environmental space’
needed for justifiable consumption increases among the poor.
7,8,9

Equal individual entitlements (quantity-based approach) would
ensure a fairer access to energy than a carbon tax (price-based
approach) under which consumers that pay more can still consume
more than the average.

The latter is the basic idea of some schemes—known as Personal
Carbon Trading—envisioning to allow the quotas received by
individuals to be traded among them. The scheme ‘Tradable Energy
Quotas’developed by the Fleming Institute in the UK is one of such
schemes. 25

A possible way of overcoming the contradictions inherent in the
tradability of permits is the use of an alternative currency for such
trade. The ‘Energy Budget Scheme’—developed by CEEweb for
Biodiversity and discussed by Veronika Kiss in the second chapter
ofthis booklet—allows the trading of permits, but only in the form
of ‘entitlement money’. This alternative currency can be used either
to pay taxes and social contributions or to buy environmentally
friendly products and services, but as such is not convertible to
legal tender money. 27

The concept of cap-and-rationing could be established for other
environmental pressures as well, such as material flows, water and
land consumption.  28

To eliminate poverty, capitalist societies generally rely on growing the
economic pie ratherthan slicing it differently.

Maximum income is essentially an income ceiling and there are
two main proposals to implement it. One suggestion is to set the
income ceiling in proportion to the minimum wage so that the
maximum wage would be, for example, twenty times the legal
minimum wage. The other suggestion is to implement a
progressive tax system, including both income and capital gains,
with a tax rate of 100% for the top tax bracket.  46 

Once basic material needs are
met, further increases in income contribute little if anything to
subjective well-being or happiness, although the steeper the social
polarisationinacountry,thebetterthe richfeel comparedtothepoor.  49

Compare against:
The Institute for Global Prosperity at University College London
developed a proposal for Universal Basic Services (UBS)
representing an affordable alternative to a Universal Basic Income
advocated by some economists.  50
}%com

\com{	cite Richard A. Warner,

"Can banks individually create money out of nothing? — The theories and the empirical evidence"

and

\href{https://professorwerner.org/category/articles-essays/}{Shifting from Central Planning to a Decentralised Economy: Do we Need Central Banks?}

and
\href{https://www.sciencedirect.com/science/article/pii/S1057521915001477}{A lost century in economics: Three theories of banking and the conclusive evidence}
}%com



==> money/princ.tex <==
\section{General Principles}

We first briefly list a number of key cross-cutting design principles that
future democratic self-organizing systems should embody,
then elaborate further below.

\begin{itemize}
\item	{\bf Completeness}:
	beyond just voting, the democratic system must address
	all the essential self-governance needs of a modern society.
\item	{\bf Simplicity}:
	all the essential principles and technological elements of the system
	should be explainable and as widely understandable as possible.
\item	{\bf Engineering}: 
	like any technology, the system must embody sound engineering practices,
	its design standing up to the careful scrutiny of leading experts.
\item	{\bf Transparency}:
	those system elements and details that not everyone can understand
	must nevertheless be open to inspection by anyone's trusted advisor.
\item	{\bf Security}:
	the system must withstand a wide variety of deliberate attacks
	from both external and internal sources,
	as well as the power of greed and self-interest.
\item	{\bf Scalability}:
	the system must support any size society robustly and efficiently
	without failure or ``help'' from vulnerable external processes.
\item	{\bf Timescales}:
	the system must operate effectively and smoothly at all timescales,
	from short-term responsiveness to immediate emergencies
	to extremely long-term, intergenerational planning and investment.
\item	{\bf Freedom}:
	the system must pervasively protect fundamental individual rights
	such as freedom of speech, association,
	and pursuit of a better life and society.
\item	{\bf Innovation}:
	the system must support, encourage, and reward entrepreneurship
	that genuinely benefits real people,
	and support innovative ventures at all scales
	while protecting smaller/newer ventures from larger/established ones.
\end{itemize}

A first key principle guiding the overal scope and organization of this work
is {\bf completeness}:
to take a ``holistic'' view on democracy,
recognizing that in practice the robust and secure functioning
of any democratic self-organizing system relies on far more
than elections, parliamentary processes, and executive bureaucracies.
To make good electoral decisions,
voters need access to reliable, trustworthy, and secure
sources of information.
To ensure widespread buy-in and resist takeover by fringe elements,
average citizens need ways to participate --
and observe direct rewards and benefits from their participation --
in ways that scale to large societies
without making unrealistic demands on the scare time of busy individuals.
To ensure that their democratic decision power makes a difference,
citizens need fair incentives to invest their time and energy
in ways that serve the needs of society as a whole and not just a small elite.
And to restore the confidence in citizens that their economic system
is fair, empowering, and sustainable,
they need a financial foundation that ensures that
money serves people instead of vice versa.
Keeping in mind that all of elements rely on each other,
subsequent sections will focus on 
the problems of information, decision-making, and economics in turn.

The goal of {\bf simplicity} -- understandability by anyone --
appears to be at odds with the principle of {\bf engineering} --
that the system must embody sound best-practice engineering principles,
which only a tiny majority of the general population
can generally be expected to know or understand.
This tension is a real and important challenge,
which we can hope to mitigate in at least three ways.
First, well-designed systems can often be made understandable by anyone
in general principles and ``broad strokes''
even if only experts can readily understand the details
of all the moving parts that make the system function.
Second, by designing a democratic system properly to encourage people to
participate in, buy into, and hence learn about the system more deeply,
we can increase the portion of the system's design
accessible to the ``average person''
and correspondingly decrease the proportion accessible only to experts.
Third, recognizing that like any complex modern technology,
a practical working democracy can never realistically be simple enough
for everyone to know and understand every operational detail,
we can rely on the principle of {\bf transparency}:
that the system be open to inspection by anyone with the requisite knowledge,
including any expert advisor who might be trusted or hired by
someone without the requisite knowledge (or time)
for a detailed inspection him/herself.

...

